Global Warming In Ghana's Major Cities Based on Statistical Analysis of NASA's POWER Over 3-Decades

Global warming's impact on high temperatures in various parts of the world has raised concerns. This study investigates long-term temperature trends in four major Ghanaian cities representing distinct climatic zones. Using NASA's Prediction of Worldwide Energy Resource (POWER) data, statistical analyses assess local climate warming and its implications. Linear regression trend analysis and eXtreme Gradient Boosting (XGBoost) machine learning predict temperature variations. Land Surface Temperature (LST) profile maps generated from the RSLab platform enhance accuracy. Results reveal local warming trends, particularly in industrialized Accra. Demographic factors aren't significant. XGBoost model's low Root Mean Square Error (RMSE) scores demonstrate effectiveness in capturing temperature patterns. Wa unexpectedly has the highest mean temperature. Estimated mean temperatures for mid-2023 are: Accra 27.86{\deg}C, Kumasi 27.15{\deg}C, Kete-Krachi 29.39{\deg}C, and Wa 30.76{\deg}C. These findings improve understanding of local climate warming for policymakers and communities, aiding climate change strategies.

==> Vita.tex <==
\section*{Vita}

\vspace{2em}

\subsection*{Personal Information}
\begin{tabular}{ll}
    \textbf{Name:} & Joshua Attih \\
    \textbf{Contact Information:} & attihjoshua@gmail.com \\
    %\textbf{Date of Birth:} & Your Date of Birth \\
\end{tabular}

\subsection*{Education}
\begin{tabular}{p{0.2\textwidth} p{0.8\textwidth}}
    \textbf{Year} & \textbf{Degree, Institution} \\
    \hline
    2017--2021 & Bachelor of Science in Physics, University of Ghana \\
    2023 & Postgraduate Diploma in Remote Sensing and GIS, UN-ARCSSTE-E, Obafemi Awolowo University \\
\end{tabular}

\subsection*{Research and Academic Achievements}
\begin{itemize}
    \item Fourier Synthesis Imaging of KAT - 7 Response to Radio Waves via Simulation; Supervised
by Prof. Nana Ama Browne Klutse, Ph.D. (South Africa);
    \item New design of a Solar Ray Collector using a cone and a parabolic cylinder as part of the
Mfano Africa-Oxford Initiative with Prof Ian Hewitt.
\end{itemize}


\subsection*{Professional Memberships}
% List any academic or professional organizations you are affiliated with.
\begin{itemize}
\item  A Student Member of the African Astronomical Society (AFAS).
    
\item Free student affiliate of the Royal Aeronautical Society (RAeS).
\end{itemize}

==> tex/acknowledgement.tex <==
\cleardoublepage
\addcontentsline{toc}{chapter}{Acknowledgement}
\chapter*{Acknowledgement}
 
I would like to thank my supervisor for  
 being able to work with my complex nature in the first place. Your ultimate support and inspiration has made this project a great success. I am so much indebted to the wealth of knowledge you provided in solving both new and old problems in all aspects related to this project work and beyond.

My sincere thanks to the United Nations for giving me a scholarship to study at their renowned ARCSSTE-E and the Nigerian Government for  providing the necessary resources to be able to kick start the project to the very end.   

Special thanks to all my friends and loved ones who have contained the hectic moments and stress I have been through during the course of this project work. 

My most thanks goes to God for giving me a wonderful mother Dzantor Kafui Evelyn who has seen me through all the various stages of my academic endeavors. 

\vspace{3em}

%Joshua ATTIH, 2023
\newpage

